Low-Rank Generalized Linear Bandit Problems

In a low-rank linear bandit problem, the reward of an action (represented by a matrix of size $d_1 \times d_2$) is the inner product between the action and an unknown low-rank matrix $\Theta^*$. We propose an algorithm based on a novel combination of online-to-confidence-set conversion~\citep{abbasi2012online} and the exponentially weighted average forecaster constructed by a covering of low-rank matrices. In $T$ rounds, our algorithm achieves $\widetilde{O}((d_1+d_2)^{3/2}\sqrt{rT})$ regret that improves upon the standard linear bandit regret bound of $\widetilde{O}(d_1d_2\sqrt{T})$ when the rank of $\Theta^*$: $r \ll \min\{d_1,d_2\}$. We also extend our algorithmic approach to the generalized linear setting to get an algorithm which enjoys a similar bound under regularity conditions on the link function. To get around the computational intractability of covering based approaches, we propose an efficient algorithm by extending the "Explore-Subspace-Then-Refine" algorithm of~\citet{jun2019bilinear}. Our efficient algorithm achieves $\widetilde{O}((d_1+d_2)^{3/2}\sqrt{rT})$ regret under a mild condition on the action set $\mathcal{X}$ and the $r$-th singular value of $\Theta^*$. Our upper bounds match the conjectured lower bound of \cite{jun2019bilinear} for a subclass of low-rank linear bandit problems. Further, we show that existing lower bounds for the sparse linear bandit problem strongly suggest that our regret bounds are unimprovable. To complement our theoretical contributions, we also conduct experiments to demonstrate that our algorithm can greatly outperform the performance of the standard linear bandit approach when $\Theta^*$ is low-rank.

==> app_algo.tex <==
In this section, we present our Low-rank Generalized Linear Bandit with Online Computation algorithm (LowGLOC).
% and the second part of LowESTR: LowOFUL algorithm in~\cite{jun2019bilinear}.
% \begin{algorithm}[h]
% 	\caption{Low-rank Generalized Linear Bandit with Online Computation (LowGLOC)}
% 	\label{algo:LowGLOC}
% 	\begin{algorithmic}
	    
% 	    \STATE \textbf{Input: }arm set: $\mathcal{X}$, horizon: $T$, $\frac{1}{T}$-net for $S_r$: $\bar{S}_r(\frac{1}{T})$, failure rate $\delta$, EW constant $\eta \asymp \frac{1}{\log\left(T/\delta\right)}$, function $m(\cdot)$ in the generalized linear model.
% 		\STATE Initial confidence set $C_0 = \{\Theta\in\mathbb{R}^{d_1\times d_2}: \left\|\Theta\right\|_F^2\leq 1\}$.
% 		\FOR{$t=1,\ldots,T$}
% 		\STATE $(X_t,\widetilde{\Theta}_t):=\argmax_{(X,\Theta)\in \mathcal{X}\times C_{t-1}} \langle X,\Theta\rangle$.
% 		\STATE Pull arm $X_t$ and receive reward $y_t$.
% 		\STATE Compute EW predictor $\hat{y}_t = \frac{\sum_{i=1}^{|\bar{S}_r(\frac{1}{T})|}e^{-\eta L_{i,t-1}}f_{\Theta_i,t}}{\sum_{j=1}^{|\bar{S}_r(\frac{1}{T})|}e^{-\eta L_{j,t-1}}}$, where $f_{\Theta_i,t} \triangleq \left\langle X_t,\Theta_i\right\rangle$ for $\Theta_i\in\bar{S}_r(\frac{1}{T})$.
% 		\STATE Update losses 
% 		$L_{i,t} = \sum_{s=1}^t-f_{\Theta_i,s}y_s+m(f_{\Theta_i,s})$, for $i=1,\ldots,|\bar{S}_r(\frac{1}{T})|$.
% 		\STATE Update $\mathcal{C}_t$ according to Equation~\ref{equ:CI_GLB}, where $B_t$ is as defined in Lemma~\ref{lemma:EW_NLL}.
% 		\ENDFOR
% 	\end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[h]
% 	\caption{LowOFUL~\citep{jun2019bilinear}}
% 	\label{algo:LowOFUL}
% 	\begin{algorithmic}
% 		\STATE \textbf{Input: }$T,k$, arm set $\mathcal{A}\subset\mathbb{R}^{d_1\times d_2}$, failure rate $\delta$ and positive constants $B,B_\perp,\lambda,\lambda_\perp$.
% 		\STATE $\Lambda = \textbf{diag}(\lambda,\ldots,\lambda,\lambda_\perp,\ldots,\lambda_\perp)$, where $\lambda$ occupies the first $k$ diagonal entries. 
% 		\FOR{$t=1,\ldots,T$}
% 		\STATE Compute $a_t = \argmax_{a\in\mathcal{A}}\max_{\theta\in \mathcal{C}_{t-1}}\langle\theta,a\rangle$.
% 		\STATE Pull arm $a_t$ and receive reward $y_t$.
% 		\STATE Update $C_t = \{\theta:\left\|\theta-\hat{\theta}\right\|_{V_t}\leq \sqrt{\beta_t}\}$, where $\sqrt{\beta_t} = \sqrt{\log\frac{|V_t|}{|\Lambda|\delta^2}}+\sqrt{\lambda}B+\sqrt{\lambda_\perp}B_\perp$, $V_t = \Lambda+\sum_{s=1}^{t}a_ta_t^T$, $\hat{\theta}_t = (\Lambda+A^TA)^{-1}A^T\mathbf{y}$. (Here $A = [a_1^T;\ldots;a_t^T]$ and $\mathbf{y}:=[y_1,\ldots,y_t]^T$).
% 		\ENDFOR
% 	\end{algorithmic}
% \end{algorithm}



==> app_complexity.tex <==
\begin{proof}
In stage 1, we solved a convex optimization problem with unknown $\Theta\in\mathbb{R}^{d_1\times d_2}$ using subgradient method, of which the complexity is $O(T_1d_1d_2/\epsilon^2)$ ($\epsilon$ refers to the target accuracy). 
The complexity of the SVD step at the end of stage 1 is $O(d_1d_2\min\{d_1,d_2\})$. 

In stage 2, Algorithm 4 (LowOFUL in Section I) dominates the computational complexity. 
In iteration $t$ of LowOFUL, $a_t = \argmax_{a\in\mathcal{A}}\max_{\theta\in\mathcal{C}_{t-1}}\langle\theta,a\rangle$ can be solved with an oracle in constant time; least square estimation takes $O(d_1^2d_2^2t+d_1^3d_2^3)$ steps. Thus, in $T_1$ iterations, the computational complexity of stage 2 is at most $O(d_1^2d_2^2T^2+d_1^3d_2^3T)$. 

Combining the complexity results in two stages, taking the target accuracy $\epsilon = 1/\sqrt{T_1}$ and $T_1 = O\left((d_1+d_2)^{3/2}\sqrt{rT}\frac{1}{\omega_r}\right)$ as stated in Theorem 4, the overall computational complexity is at most $O\left(d_1^2d_2^2T^2\right)$ for sufficiently large $T$.
\end{proof}


==> application.tex <==
\subsection{Causal Bandits Setup}
A directed acyclic graph $\mathcal{G}$ is used to model the causal structure over a set of random variables $\mathcal{X} = \{X_1,\ldots,X_N\}$. $P$ is the joint distribution over $\mathcal{X}$ that factorizes over $\mathcal{G}$. 
We assume each variable only takes on $k$ distinct values. The parents of a variable $X_i$, denoted by $\text{Pa}_{X_i}$, is the set of all variables $X_j$ such that there is an edge from $X_j$ to $X_i$ in $\mathcal{G}$. 
A size $m$ intervention (action) is denoted by $do(\mathbf{X} = \mathbf{x})$, which assigns the values $\mathbf{x} = \{x_1,\ldots,x_m\}$ to the corresponding variables $\mathbf{X} = \{X_1,\ldots,X_m\} \subset \mathcal{X}$. 
An empty intervention is $\text{do}()$. 
The intervention on $\mathbf{X}$ also removes all edges from $\text{Pa}_{X_i}$ to $X_i$ for each $X_i \in \mathbf{X}$. 
Thus the resulting underlying probability distribution that defines the graph is denoted by $P(\mathbf{X}^c|do(\mathbf{X}=\mathbf{x}))$ over $\mathbf{X}^c:= \mathcal{X}-\mathbf{X}$.

In this causal bandit problem, the reward variable $Y$ is real-valued. 
A learner is given the causal model's graph $\mathcal{G}$\footnote{Even though our algorithms take $\mathcal{G}$ as input, the only information used is the identity of $\text{Pa}_Y$ variables.}, a set of interventions (actions) $\mathcal{A}$.
%and conditional distributions of parent variables of $Y$ given an intervention $a \in \mathcal{A}$: $P(\text{Pa}_Y|a)$. 
We denote the expected reward for action $a = \text{do}(\mathbf{X}=\mathbf{x})$ by $\mu_a:= \mathbb{E}\left[Y|\text{do}(\mathbf{X}=\mathbf{x})\right]$. The optimal action is defined as $a^* := \argmax_{a\in \mathcal{A}}\mu_a$. 
We assume $\mu_a \in [0,1]$ for every $a \in \mathcal{A}$. In round $t$, the learner pulls $a_t = \text{do}(\mathbf{X}_t=\mathbf{x}_t)$ based on previous round knowledge and causal information, then observes the reward $Y_t$ and the values of $\text{Pa}_Y$, denoted by $\mathbf{Z}_{(t)} = \{z_1(t),\ldots,z_n(t)\}$, where $n$ is the number of reward's parent variables. 

One can then write $\mu_a = \sum_{\mathbf{Z}}P(\text{Pa}_Y=\mathbf{Z}|a)\mathbb{E}\left[Y|\text{Pa}_Y=\mathbf{Z}\right]$ and \citep{lu2019regret} proposed causal UCB and causal TS algorithms that only achieve regret $\tilde{O}\left(\sqrt{|\mathbf{Z}|T}\right)$ instead of $\tilde{O}\left(\sqrt{|\mathcal{A}|T}\right)$. Their algorithm crucially depends on the knowledge of $P(\text{Pa}_Y=\mathbf{Z}|a)$ for all $\mathbf{Z}$ and $a$. However, in certain cases, these conditional probabilities are hard to obtain. We will consider several ways to model this quantity and see how this approach can be related to low rank bandit.

\subsection{Model 1: Linear  Reward Model}
\begin{assumption}[Linear reward]
	For given parent variables $\mathbf{Z}$, there exists a vector $\omega^*\in\mathbb{R}^{d_2}$ and feature vectors $\varphi(\mathbf{Z})$ such that
	\begin{align}
	Y = \varphi(\mathbf{Z})^T\omega^*+\epsilon,
	\end{align}
	where $\epsilon$ is subgaussian 1 error and $\left\|\omega^*\right\|_2\leq 1$.
\end{assumption}
\begin{assumption}[Linear modeling for conditional probabilities]
	For each $a\in\mathcal{A}$ and $\mathbf{Z}\in\mathcal{Z}$, where $\mathcal{Z}$ is the set of all value combinations of reward's parent nodes, feature vectors $\phi(\mathbf{Z},a)$ are given as a priori. There exists a vector $\theta^*\in\mathbb{R}^{d_1}$, such that
	\begin{align}
	P(\text{Pa}_Y=\mathbf{Z}|a) = \phi(\mathbf{Z},a)^T\theta^*.
	\end{align}
	Here we assume $\left\|\theta^*\right\|\leq 1$ and $\left\|\phi(\mathbf{Z},a)\right\|\leq 1$, for all $a\in\mathcal{A}$ and $\mathbf{Z}\in\mathcal{Z}$.
\end{assumption}



We can write the expected reward for every action $a\in\mathcal{A}$ as:
\begin{align}
\mu_a &= \sum_{j=1}^{k^n} P(\text{Pa}_Y = \mathbf{Z}_j|a)\varphi(\mathbf{Z}_j)^T\omega^*\\
&= \sum_{j=1}^{k^n} \phi(\mathbf{Z}_j,a)^T\theta^*\varphi(\mathbf{Z}_j)^T\omega^*\\
&= \sum_{j=1}^{k^n}\langle \phi(\mathbf{Z}_j,a)\varphi(\mathbf{Z}_j)^T,\theta^*\omega^{*T}\rangle\\
&= \langle \sum_{j=1}^{k^n}\phi(\mathbf{Z}_j,a)\varphi(\mathbf{Z}_j)^T,\theta^*\omega^{*T}\rangle.
\end{align}
Thus we can view $\sum_{j=1}^{k^n}\phi(\mathbf{Z}_j,a)\varphi(\mathbf{Z}_j)^T$ as the feature for action $a$, and $\theta^*\omega^{*T}$ works as a $d_1\times d_2$ rank 1 linear coefficient.

Using exponential weighting averaged forcaster method or explore-then-refine by assuming RSC condition, one can achieve regret that is, $\tilde{O}\left((d_1+d_2)^{3/2}\sqrt{T}\right)$, while the naive approach scales with $\tilde{O}\left(d_1d_2\sqrt{T}\right)$.

\subsection{Model 2: Additive Linear Reward Model}
\begin{assumption}[Additive Linear Rewards]
	Suppose the given parent variables $\mathbf{Z}$ can be categorized into $K$ groups: $\mathbf{Z}_1,\ldots,\mathbf{Z}_K$, there exists vectors $\omega_1^*,\ldots,\omega_K^*\in\mathbb{R}^{d_2}$ and features $\varphi(\mathbf{Z}_1),\ldots,\varphi(\mathbf{Z}_1)\in\mathbb{R}^{d_2}$ such that
	\begin{align}
		Y = \varphi(\mathbf{Z}_1)^T\omega_1^*+\ldots+\varphi(\mathbf{Z}_1)^T\omega_K^*+\varepsilon,
	\end{align}
	where $\varepsilon$ is a subgaussian-1 error term and $\left\|\varphi(\mathbf{Z}_i)\right\|_2\leq 1, \left\|\omega_i^*\right\|_2\leq 1$ for all $i\in[K]$ and $\mathbb{Z}_i$.
\end{assumption}

\begin{assumption}[Conditional Independent Parent Groups of Reward]
	For each action $a\in\mathcal{A}$ and parents $\mathbf{Z}\in\mathcal{Z}$ grouped into $\mathbf{Z}_1,\ldots,\mathbf{Z}_K$, we have
	\begin{align}
		\mathbb{P}(\mathbf{Z}_1,\ldots,\mathbf{Z}_K|a) = \prod_{i=1}^K\mathbb{P}(\mathbf{Z}_i|a).
	\end{align}
\end{assumption}

\begin{assumption}[Group linear modeling for conditional probabilities]
	For each action $a\in\mathcal{A}$ and parents $\mathbf{Z}\in\mathcal{Z}$ grouped into $\mathbf{Z}_1,\ldots,\mathbf{Z}_K$, there exists vectors $\theta_1^*,\ldots,\theta_K^*\in\mathbb{R}^{d_1}$ and features $\phi(\mathbf{Z}_1,a),\ldots,\phi(\mathbf{Z}_K,a)\in\mathbb{R}^{d_1}$ such that
	\begin{align}
		\mathbb{P}(\mathbf{Z}_i|a) = \phi(\mathbf{Z}_i,a)^T\theta_i^*,
	\end{align}
	where $\left\|\phi(\mathbf{Z}_i,a)\right\|_2\leq 1$ and $\left\|\theta_i^*\right\|_2\leq 1$ for all $i\in[K]$ and $(\mathbf{Z}_i,a)$ pairs.
\end{assumption}

Under above assumptions for additive linear reward model, the expected reward for every action $a\in\mathcal{A}$ can be written as
\begin{align}
	\mu_a &= \mathbb{E}\left[Y|a\right]\\
	&= \sum_{\mathbf{Z}_1}\cdots\sum_{\mathbf{Z}_K}\mathbb{P}(\mathbf{Z}_1,\ldots,\mathbf{Z}_K|a)\mathbb{E}\left[Y|\mathbf{Z_1},\ldots,\mathbf{Z}_K\right]\\
	&=\sum_{\mathbf{Z}_1}\cdots\sum_{\mathbf{Z}_K}\prod_{i=1}^K\mathbb{P}(\mathbf{Z}_i|a)\sum_{j=1}^{K}\varphi(\mathbf{Z}_j)^T\theta_j^*\\
	&= \sum_{i=1}^K\sum_{\mathbf{Z}_i}\mathbb{P}(\mathbf{Z}_i|a)\varphi(\mathbf{Z}_i)^T\theta_i^*\\
	&=\sum_{i=1}^K\sum_{\mathbf{Z}_i}\phi(\mathbf{Z}_i,a)^T\omega_i\varphi(\mathbf{Z}_i)^T\theta_i^*\\
	&=\langle \sum_{\mathbf{Z}_1}\phi(\mathbf{Z}_1,a)\varphi(\mathbf{Z}_1)^T,\omega_1^*\theta_1^{*T}\rangle+\ldots+\langle \sum_{\mathbf{Z}_K}\phi(\mathbf{Z}_K,a)\varphi(\mathbf{Z}_K)^T,\omega_K^*\theta_K^{*T}\rangle\\
	&=\langle\left[B_1 \cdots B_K\right],\left[\omega_1^*\theta_1^{*T} \cdots \omega_K^*\theta_K^{*T}\right]\rangle,
\end{align}
where $B_i:=\sum_{\mathbf{Z}_i}\phi(\mathbf{Z}_i,a)\varphi(\mathbf{Z}_i)^T\in\mathbb{R}^{d_1\times d_2}$, and we use $\left[B_1 \cdots B_K\right]\in\mathbb{R}^{d_1\times d_2 K}$ and $\left[\omega_1^*\theta_1^{*T} \cdots \omega_K^*\theta_K^{*T}\right]\in\mathbb{R}^{d_1\times d_2K}$ to denote the concatenated matrices.

Since $\{w_i^*\theta_i^{*T}\}_{i=1}^K$ are $K$ rank-1 matrices, the rank of concatenated matrix  $\left[\omega_1^*\theta_1^{*T} \cdots \omega_K^*\theta_K^{*T}\right]\in\mathbb{R}^{d_1\times d_2K}$ is at most $K$.

Naive linear bandit approach on this problem has $\widetilde{O}\left(d_1d_2K\sqrt{T}\right)$ regret, but both our efficient and inefficient approaches only have $\widetilde{O}\left((d_1+d_2K)^{3/2}\sqrt{KT}\right)$. This is a big improvement since usually $d\gg K$.
